Learning from the Worst: Dynamically Generated Datasets to Improve Online Hate Detection

We present a human-and-model-in-the-loop process for dynamically generating datasets and training better performing and more robust hate detection models. We provide a new dataset of ~40,000 entries, generated and labelled by trained annotators over four rounds of dynamic data creation. It includes ~15,000 challenging perturbations and each hateful entry has fine-grained labels for the type and target of hate. Hateful entries make up 54% of the dataset, which is substantially higher than comparable datasets. We show that model performance is substantially improved using this approach. Models trained on later rounds of data collection perform better on test sets and are harder for annotators to trick. They also perform better on HateCheck, a suite of functional tests for online hate detection. We provide the code, dataset and annotation guidelines for other researchers to use. Accepted at ACL 2021.

==> reviewerResponse.tex <==

%%%% OUR RESPONSE %%%%%

\section{Submit Response to Reviewers}
%Use the following boxes to enter your response to the reviews. Please limit the total amount of words in your comments to 1000 words (longer responses will not be accepted by the system).

\subsection{Response to Review #1, 4}
Thank you for these comments.

\subsection{Response to Review #2, 4}
%Were the unrealistic examples in "Section 5 Lessons from R2 (line 480-481)" included in the dataset?
Unrealistic examples. We removed the unrealistic examples from the dataset, as well as the majority of uses of templates. 

Model performance on R0. We have not evaluated M1 to M4 against R0. Our analyses (and the low performance of M1) indicate that it contains lots of non-relevant and noisy data. This is also shown in several recent papers (https://d-nb.info/1190084805/34 and https://link.springer.com/article/10.1007/s10579-020-09502-8). We are concerned that the quality of R0 means it could be an unhelpful comparison point.



Why were the different types of hate not noted in r1 (Table 1)?
It was not recorded. A benefit of our method is that as annotators learn and improve the annotation categories can be updated to reflect how their knowledge and understanding of the task develops. 

HateCheck. This is a good point, and HateCheck outlines it should only be used to test, not train. None of the entries are direct matches. However, we will investigate this further and if we find evidence of overlap flag this appropriately in our results. 


Impact of upsampling. Table 4 shows both target model performance and the scores for models trained on equal weightings of the data. M3 achieves 75.48 accuracy, comparing to 74.53 on an equal weighting of R0, R1 and R2. This suggests that upsampling drives a modest improvement in performance. 

Annotator biases. We are aware of the risk of annotator biases. The task of generating hateful and non-hateful (but relevant) content is likely to also generate a small set of content that has a high similarity due to a limited number of stereotypes and tropes being used in real world settings to be hateful. As per your suggestion we will analyse similarity of entries from different annotators.
%One of the concerns will be about similar kind of content from different annotators. I found a few samples in the dataset which were similar but done by different annotators. This can also increase the model performance. Can the authors address this concern in the final version of the dataset (by running some similarity metric)?

Standard deviation across the 5 training seeds. We will include this in the CR if accepted.
%What are the standard deviation across five training seeds?

Other. We will update line 483 to address the phrasing. Thanks.




\subsection{Response to Review #3, 3.5}

Labelling schema. We developed the labeling schema based on our prior work and other taxonomies. We also reviewed a large amount of soc sci literature. We will use extra space to report this work, including drawing on the papers you recommended. We will also include a better justification of our definition of online hate.
Specifically, we used the work of Davidson, Waseem, Zampieri and Vidgen (et al.) to identify relevant categories. We split animosity and derogation in line with work that separates implicit hate from explicit. We deviated from previous taxonomies because (1) threatening language is a very harmful form of hate, but is rarely distinguished in taxonomies (see Anzovino's 2018 misogyny task and Golbeck's 2017 harassment corpus for exceptions), (2) glorification of hateful entities and (3) dehumanization are important for understanding how online hate is expressed, yet are also often not separated.

Introduction of new forms of bias. We are concerned about this and so (a) hold out some annotators for test sets and (b) tasked annotators to look at real-world content in r3 and r4. We plan on exploring this in future work. 
%However, I am worried about the feasibility of the task and whether it may create another form of bias (despite countering label bias due to key-phrases), especially after I checked the data. In addition, the evaluation does not show whether this method is adapted to multi-class classification tasks or robustness. (See questions)

Model performance.
We will provide F1 scores alongside accuracy in the paper. Both metrics are useful, but we agree F1 would help better substantiate our claims of improved performance + robustness. 
%In the case of fine-grained classification tasks, the accuracy does not prove that the model performs better and does not tell us whether the model is more robust or not (even if intuitively, the idea that is presented in this paper should improve the robustness of the model). Reporting F1 scores would have been better (for the sake of comparison, even if the authors reported error rates).

Perturbations. The suggestion of bias from too many perturbations is interesting. We will evaluate this, incl. models trained on only originals, tested on perturbations (and vice versa). 
%My main question is how do you think you can counter possible bias that can be introduced from "too many" perturbations?

Extensions of the work. The process we outline utilizes the dynabench platform, and is open to new tasks.%It includes as sentiment model, who are taking a somewhat similar approach to us.
In principle, our approach could be used for multi-class hate detection, we can add this to the discussion. % although it may be more difficult to ensure uniform coverage of classes.



\subsection{Response to Review #4, 4.5}
What drives the increased performance?
Table 4 shows both target model performance and the scores for models trained on equal weightings of the data. For example: M3 achieves 75.48 accuracy, comparing to 74.53 on an equal weighting of R0, R1 and R2. This suggests that upsampling drives a modest improvement in performance. 
We follow your proposal of fixing the upsampling factor at the end of each round. We will clarify in the CR paper, if accepted. %This means we do not fully optimize performance in each round, but have 'cumulative' model development. We will explain this more clearly in the CR paper if accepted.
%Is the increased performance of, e.g,, M2 vs M(R0+R1) because of the cumulative training or because of the upsampling of the data? I’m not sure what else is different between these two.  It seems that maybe a different way to learn these models is to split the data into R0,R1,R2,R3,R4 and then tune the upsampling factor of each (in sequence, fixing the best value for each one at a time). Is this what is meant by cumulative learning, or am I missing something about how this works? Maybe there would be a way to present this more clearly in Table 4, currently it is difficult to clearly understand the precise differences between the first 4 and last 4 columns.


Did you consider other tests of generalization? 
We did, but they are not included for space. Space permitting, we would aim to include in the appendix.
%Did you consider any other tests of generalization? E.g., hold out one training set from R0 and use it as a test set (with no training on data from that set). This might highlight the strengths of this approach even more.

Annotator recruitment and guidelines. We recruited annotators through our networks. Information about annotators is given in our supplementary materials in our data statement. Annotation guidelines are to be shared publicly. 

Are the categories of hate mutually exclusive? Yes, i.e. each hateful entry can only be one of animosity, dehumanization, derogation, support for hateful entities and threatening.

Why 4 steps? We drew on https://arxiv.org/abs/1908.06083, who used 3 rounds of 1k for creating a safe chatbot. We planned for rounds to increase in sophistication.

Real-world content inspiration. We gave explicit instructions to annotators that no original content must be entered. We held 'explainer' sessions, giving them examples and talking through what counts as a sufficient change. At the start we had annotators send us examples of their changes and gave them feedback.

Other: We will include the missing references for line 235.

%How do we keep it up to date? We are currently exploring this with our future rounds of data collection, including creation of smaller rounds to address more niche issues, such as how emojis are used to express hate. 


\subsection{General Response to Reviewers}
Thank you for these comments and engaging so thoroughly with our work. 


\subsection{Response to Chairs} % NONE

%Use this textbox to contact the chairs (including area chair and senior area chairs) directly only when there are serious issues regarding the reviews. Such issues can include reviewers who grossly misunderstood the submission, or have made unfair comparisons or requests in their reviews. Most submissions should not need to use this facility.









\section{Reviews}
\subsection{Review #1}
The core review
The paper presents a human-and-model-in-the-loop process that was employed to collect a series of large scale dynamically generated hate speech datasets.
Overall, the paper is well-written and it has good contribution in the field, however, it was better if the authors have provided a flowchart showing the overall process.

No Appendix is provided in the paper as the authors have mentioned several times which makes some parts not easy to understand.

Reasons to Accept
The paper provides a decent approach in dynamic dataset generation.
Overall Recommendation:	4



\subsection{Review #2}
The core review
Hate speech datasets are often static in nature. This static form of hate speech dataset is not good for evaluation as language dynamics in online social media changes rapidly. This paper lays the foundation for a dynamic benchmark for hate speech dataset in a human in the loop setting. Here the annotators are asked to produce different types of hate speech in order to make the model predict wrong. The subsequent rounds use the datasets where the model went wrong and use it to train the models better. The evaluation with hate check may be confounding as the templates for fooling the models are similar to hatecheck functionalities.

Reasons to Accept
The proposed method of data collection and model training with a human-in-the-loop framework is important for complex tasks like Hate speech/ sarcasm detection

The authors have taken adequate steps to make the data diverse with a limited set of annotators.
The annotation guidelines are detailed and useful for future research in hate speech

Reasons to Reject
Some of the sections are not clearly written
For the 1st round accuracy does not seem a correct metric for comparison.

Overall Recommendation:	4
Questions for the Author(s)
Were the unrealistic examples in "Section 5 Lessons from R2 (line 480-481)" included in the dataset?
What is the performance of the model if it is trained on R1 to R4 (synthetic data) and tested on R0?
Why were the different types of hate not noted in Round 1 (Table 1)?
Is it possible that many of the templates from Round 2 were actually part of the functionality tests in Hatecheck, thereby increasing the performance?
Did the authors check how much the performance dropped without the upsampling (343-345)?
One of the concerns will be about similar kind of content from different annotators. I found a few samples in the dataset which were similar but done by different annotators. This can also increase the model performance. Can the authors address this concern in the final version of the dataset (by running some similarity metric)?
What are the standard deviation across five training seeds?
Typos, Grammar, Style, and Presentation Improvements
In line 483, I guess the authors wanted to mean "small" instead of "large"



\subsection{Review #3}
The core review
The paper presents a methodology to build robust hate speech classifiers with human annotators involved in the process. It also introduces a new fine-grained dataset collected within 4 rounds. The annotators tricked the model with challenging "perturbated" entries to counter the inherent bias of hate speech classifiers. The paper reports that this method improved the robustness of the model.
Building robust hate speech classifiers is challenging and important, this work's main claim is useful and could be extended.

However, I am worried about the feasibility of the task and whether it may create another form of bias (despite countering label bias due to key-phrases), especially after I checked the data. In addition, the evaluation does not show whether this method is adapted to multi-class classification tasks or robustness. (See questions)

Reasons to Accept
The paper is well written, the methodology is coherent, and I believe that it can be part of an online moderation process. I also believe that it would be useful for building new hate speech datasets, updating, or improving the quality of available hate speech datasets.

The idea can even be extended to other tasks such as sentiment analysis datasets that suffer from selection bias.

The annotation process is interesting.

Reasons to Reject
The motivation behind using this labeling schema is not clear and the authors did not compare it to other available labeling schemas (such as those involving hate intensity). Indeed, there is no unanimous definition of hate speech but the authors do not justify their choice.

In the case of fine-grained classification tasks, the accuracy does not prove that the model performs better and does not tell us whether the model is more robust or not (even if intuitively, the idea that is presented in this paper should improve the robustness of the model). Reporting F1 scores would have been better (for the sake of comparison, even if the authors reported error rates).

Overall Recommendation:	3.5
Questions for the Author(s)
My main question is how do you think you can counter possible bias that can be introduced from "too many" perturbations?
Do you have F-score results?

You can add a subsection to the related work and compare your annotation schema to other annotation schemas.

Missing References
Examples of papers with hate speech targets + relevant to your labeling schema:
ElSherief, Mai, et al. "Hate lingo: A target-based linguistic analysis of hate speech in social media." Proceedings of the International AAAI Conference on Web and Social Media. Vol. 12. No. 1. 2018.

Fortuna, Paula, et al. "A hierarchically-labeled Portuguese hate speech dataset." Proceedings of the Third Workshop on Abusive Language Online. 2019.

Ousidhoum, Nedjma, et al. "Multilingual and multi-aspect hate speech analysis." Proceedings of EMNLP. 2019.

Sap, Maarten, et al. "Social bias frames: Reasoning about social and power implications of language." Proceedings of ACL. 2020.

This paper is also relevant since they introduced hate intensity:

Sanguinetti, Manuela, et al. "An Italian Twitter corpus of hate speech against immigrants." Proceedings of the Eleventh International Conference on Language Resources and Evaluation (LREC 2018). 2018.



\subsection{Review #4}
The core review
In this paper, the authors present a 4-round human-in-the-loop dynamic adversarial dataset generation process for hate detection. They start with a large set of existing hate datasets and train a RoBERTa model on these. Then, they ask humans to generate new difficult examples for this model using a variety of tactics depending on the round, and re-train the model after each round to make it more difficult to trick. The resulting model after the fourth round shows good performance on the HATECHECK benchmark.
The authors took a lot of care to make sure the process was done in a reasonable way and that annotators were well trained and monitored along the way. The paper is easy to follow and this approach makes sense. With the release of the data and pre-trained models, I can see this work being beneficial to the ACL community and helping to fuel future studies on online hate detection.

As with other similar datasets, I am not sure if this work addresses the fact that what is considered hate and the ways in which hate are expressed can change over time. How useful will this dataset/model be in 1, 5, or 10 years? That may be out of the scope of this paper, but the method does require a lot of human effort and so it might be difficult to repeat to keep models up-to-date. However, the way the approach works might actually lend itself well to this situation, since each model is built on top of the previous ones, perhaps this means only one new step will be needed each time instead of all 4.

Reasons to Accept
Well documented approach could be useful for the creation of other datasets

The resulting models and datasets should be useful for hate detection research in general

Brings attention to an important research topic with potential for positive societal impact

Reasons to Reject
More details about annotator guidelines will be needed to make this more reproducible in the case that models need to be updated or applied to other tasks
Overall Recommendation:	4.5
Questions for the Author(s)
Are the categories of hate mutually exclusive?
It would be helpful to have a clear unified definition of Hate as it is used in this paper early on since it seems to be more specific than the general meaning of “hate” (as suggested by the capitalization). In section 3, the Warner and Hirschberg definition is used, but other refinements are added later, e.g., it must target a vulnerable, marginalized or discriminated-against group.

How were the annotators recruited? What were the guidelines provided to them?

In the later rounds, where annotators used real-world content to inspire them, how much paraphrasing/modification was required? Was there any check done to ensure that the new text was substantially different from the original and might this have any effect on the models’ ability to generalize?

Is the increased performance of, e.g,, M2 vs M(R0+R1) because of the cumulative training or because of the upsampling of the data? I’m not sure what else is different between these two. It seems that maybe a different way to learn these models is to split the data into R0,R1,R2,R3,R4 and then tune the upsampling factor of each (in sequence, fixing the best value for each one at a time). Is this what is meant by cumulative learning, or am I missing something about how this works? Maybe there would be a way to present this more clearly in Table 4, currently it is difficult to clearly understand the precise differences between the first 4 and last 4 columns.

Did you consider any other tests of generalization? E.g., hold out one training set from R0 and use it as a test set (with no training on data from that set). This might highlight the strengths of this approach even more.

How did you determine that 4 steps was enough? Why not 5? Why these 4 steps in this particular sequence?

Missing References
Can you include references for the claim on line 235 beginning “Previous research shows…”?
Typos, Grammar, Style, and Presentation Improvements
(see questions above re: Table 4)





\section{Things to improve in the future}
%%% BIGGER POINTS %%%
1. Is accuracy the correct score, instead of F1 (r2, r3)?
2. How do we handle the dodgy templates... they were excluded I think? 
3. Responding to the taxonomy design, and comparing it against previous efforts.
4. Robustness, i.e. the impact of perturbations (r3), future relevance/quality (r4).

%% ACTIONS %%



